Faster Combinatorial k-Clique Algorithms

Detecting if a graph contains a $k$-Clique is one of the most fundamental problems in computer science. The asymptotically fastest algorithm runs in time $O(n^{\omega k/3})$, where $\omega$ is the exponent of Boolean matrix multiplication. To date, this is the only technique capable of beating the trivial $O(n^k)$ bound by a polynomial factor. Due to this technique's various limitations, much effort has gone into designing "combinatorial" algorithms that improve over exhaustive search via other techniques. The first contribution of this work is a faster combinatorial algorithm for $k$-Clique, improving Vassilevska's bound of $O(n^{k}/\log^{k-1}{n})$ by two log factors. Technically, our main result is a new reduction from $k$-Clique to Triangle detection that exploits the same divide-and-conquer at the core of recent combinatorial algorithms by Chan (SODA'15) and Yu (ICALP'15). Our second contribution is exploiting combinatorial techniques to improve the state-of-the-art (even of non-combinatorial algorithms) for generalizations of the $k$-Clique problem. In particular, we give the first $o(n^k)$ algorithm for $k$-clique in hypergraphs and an $O(n^3/\log^{2.25}{n} + t)$ algorithm for listing $t$ triangles in a graph.

==> technical-overview.tex <==
% !TEX root = ../main.tex
\section{Technical overview of previous works} \label{sec:technical-overview}

\nick{Sorry, I only now got to read this section. Unfortunately, I think that it's way too elaborate. I agree that it makes sense to quickly mention how Four-Russians works, but not more than just a paragraph. For all the other previous work I think a single sentence would be sufficient. And even if we decide to include this, I think this is not an appropriate place---after all, we want the readers to learn about our work and not about the work of others.}
\amir{Re placement - it can be a subsection of the prelims (at the end). Re length/detail I agree - yarin, the current version can be put in a literature review section in your thesis; let's try to make a short version of 1-2 sentences per technique (I can do it quickly later too).}

We provide an overview of the previous bodies of work on the topic mentioned in the introduction and the algorithmic techniques these works employ. Although most of these results were formulated as BMM algorithms, we reformulate the ideas for the triangle detection problem why is more fitting in the current context.

\subsection{The Four-Russians method}
We start with presenting the most basic form of the Four-Russians method, and then move on to a specific variant which we will use throughout this paper. In the Four-Russians method, we start by precomputing the solutions for triangle detection on tiny instances. In particular, we precompute and store the solution to triangle detection on every tri-partite graph with vertex sets of size $s\in O\left(\sqrt{\log(n)}\right)$ and store the answers in a lookup table. Then, we use this precomputation to accelerate triangle detection on the input graph: We partition every vertex set in the input graph into blocks of size $s$. Then, for each triplet of blocks we query the lookup table with the subgraph induced by the triplet to obtain an answer to whether there exists a triangle among these blocks. Assuming a word-RAM model with $w\in\Omega\left(\log(n)\right)$, and some additional preprocessing which allows to determine subgraphs on combinations of blocks efficiently, the running time is dominated by the number of queries to the lookup table which is $O\left(\frac{n^3}{\log^{1.5}(n)}\right)$. To present the specific variant we use, which achieves slightly better running times: Given a tri-partite graph $G=\left(\left(V_{1},V_{2},V_{3}\right),E\right)$, we begin by preprocessing the graph: We divide $V_{2}$ and $V_{3}$ into blocks of size $\varepsilon\cdot\log\left(n\right)$ for some small $\varepsilon>0$. Now, for every pair of the form $\left(S,S'\right)$ where $S$ is a subset of a block in $V_{2}$ and $S'$ is a subset of a block in $V_{3}$, we check whether there exists an edge between the two sets and store the answer in a lookup table. This preprocessing is efficient: each block has $O\left(n^{\varepsilon}\right)$ subsets and the number of blocks in each vertex set is at most $O\left(\frac{n}{\log(n)}\right)$. This means the total number of pairs $\left(S,S'\right)$ is at most $O\left(\frac{n^{2+2\varepsilon}}{\log^{2}(n)}\right)$. Since we spend logarithmic time for each pair, the preprocessing time is truly subcubic. This preprocessing allows accelerating triangle detection: For each $v\in V_{1}$, we partition the neighbourhood of $v$ in $V_{2}$ into subsets of blocks, and do the same for the neighbourhood of $v$ in $V_{3}$. Now, for every combination of subsets of neighbours, query the lookup table. If the answer to any query is YES, it means that there exists an edge between two neighbours of $v$ which implies the existence of a triangle. For each vertex we spend $O\left(n\right)$ in partitioning the neighbourhoods, and then perform $O\left(\frac{n^{2}}{\log^{2}\left(n\right)}\right)$ queries to the lookup table. Assuming a word-RAM model with $w\in\Omega\left(\log\left(n\right)\right)$, queries to the lookup table can be performed in constant time. So, the total running time becomes $O\left(\frac{n^{3}}{log^{2}\left(n\right)}\right)$. Note that this technique can also be used to list all triangles in the graph: Instead of storing YES or NO in the lookup table as to whether there exists an edge between the two sets, we can store a list of all edges between the sets, and then use these lists when performing queries - this would add a cost of $O(t)$ to the running time where $t$ is the number of triangles in the graph. Vassilevska \cite{Vassilevska09Clique} demonstrated how the Four-Russians technique can be used for $k$-clique in a similar fashion: $V_2,...,V_k$ are each partitioned into blocks and for every $(k-1)$-tuple of blocks the answer to whether there exists a $(k-1)$-clique amongst the blocks is stored in a lookup table.

\subsection{Bansal and Williams' use of regularity lemmas}
Bansal and Williams \cite{BansalW12} employed regularity lemmas for triangle detection. We can think about the role regularity plays for triangle detection intuitively: The density of two sets $(S,T)$ refers to the ratio of the number of edges crossing $S$ and $T$ to the number of pairs $(s,t)\in S\times T$, so dense sets have many edges (compared to the complete bipartite on these sets). Saying $(S,T)$ is a regular pair, means large subsets of $S$ and $T$ have approximately the same density as $S$ and $T$. This means if $(S,T)$ is a dense, regular pair, then large subsets of $S$ and $T$ must be connected by an edge. This brings us to triangle detection - if we have a regular partition on $(V_2,V_3)$ (a partition in which largely every two pieces are regular), we can divide the triangle detection instance into two subproblems. One subproblem is a subgraph with only edges connecting small density partition pieces between $V_2$ and $V_3$ - such a graph has by definition few edges which makes triangle detection easier. The other subproblem only has edges between large partition pieces. Then, looking at a vertex $v\in V_1$ and a pair of partition pieces in $V_2$ and $V_3$, if $v$ does not have many neighbors within these partition pieces we can check if there exists an edge between the neighbors efficiently. Otherwise there are many neighbours, and large sets of neighbors between dense regular pairs means there must exist an edge between them - this exposes a triangle. To surpass the running time of the Four-Russians method, Bansal and Williams combined regularity lemmas with alterations to the standard Four-Russian technique - an important technical contribution. In more detail, they observed that the Four-Russians method can be altered in a way that compounds sparseness in the graph with the $\log^2(n)$ factor shaved by the standard technique. In essence, what this means, is that in a tri-partite graph in which $\sum_{v\in V_{1}}d_{2}\left(v\right)\cdot d_{3}\left(v\right)\leq\alpha\cdot n^{2}$ for some fraction $\alpha$ that is atleast $1/polylog$, we can achieve a running time of $O\left(\frac{n^{3}}{\alpha\cdot log^{2}\left(n\right)}\right)$ for combinatorial triangle detection(see \cref{lem:sparse-four-russians}).


%This observation gave rise to two algorithms that achieve faster running times than the standard method. The %first algorithm uses a triangle removal lemma. In short, we use random sampling to detect the existence of a %triangle in the graph. If the graph has many triangles, this step succeeds with high probability. Otherwise, %the graph has few triangles, and so a removal lemma can be used to obtain a set of $o\left(n^2\right)$ edges %such that every triangle in the graph uses some edge in the set. This allows us to solve the problem on %sparser subgraphs and go beyond $\log^2(n)$ shaving. The second algorithm uses pseudoregularity, and is %presented in \cref{sec:triangle-listing}.

\amir{you should mention the high level point explaining why regularity makes sense: dense and regular graphs must have triangles.}
\yarin{I did, I worry this may be too detailed/long what do you think? Also, there is some background I provide later about pseudoregularity, because we use it directly. It is a bit strange that the background appears later, but also here I talk about regularity in Szemerdi's sense, and I have no reason to give background for it because it's never directly used in the paper...}
\amir{yeah it's longer and more detailed than i imagined... but it's OK}

\subsection{Chan's use of divide-and-conquer techniques}
Chan's \cite{Chan15} main observation was that if there is some high-degree node, we can check its neighbors for the existence of an edge (such an edge exists if and only if the vertex is involved in a triangle), and recurse on significantly smaller subproblems which do not contain these (large) neighborhoods. We can continue to recurse until we reach a graph in which all vertices have small degrees, i.e a sparse graph, and then compound this sparseness with the $\log^2{n}$ gained from the standard technique. An analysis shows that the overhead involved in recursion is quite small, and the running time is dominated by the sparse instances. Chan showed a running time of $\Ologlog\left(\frac{n^3}{\log^3(n)}\right)$ can be achieved. Yu \cite{Yu18} later expanded this result to show such techniques can be used to achieve a running time of $\Ologlog\left(\frac{n^3}{\log^4(n)}\right)$.

